Lorenzen's reshaping of Krull's Fundamentalsatz for integral domains (1938--1953)

Krull's Fundamentalsatz, the generalisation of the main theorem of elementary number theory to integral domains, is the starting point of Lorenzen's career in mathematics. This article traces a conceptual history of Lorenzen's successive reformulations of the Fundamentalsatz on the basis of excerpts of his articles. An edition of the extant correspondence of Lorenzen with Hasse, Krull, and Aubert provides a better understanding of the context of these investigations.

==> 19530514-PL-1-1-87-Lorenzen-Hasse <==
\hfill[PL~1-1-87]

\hfill Bonn, den 14.5.53\hspace*{3em}

Sehr verehrter, lieber Herr Hasse,

aus Freude und Dankbarkeit darüber, dass Sie in Ihrem Vor\bs
trag über Mathematik als Wissenschaft, Kunst und Macht
auch einmal die menschliche Seite der Mathematik --\nbsp
die Empfindungen und Beweggründe, die uns gerade an diese
Wissenschaft vor allen anderen binden (obwohl Sie betonen,
dass Sie nur Ihre subjektive Einstellung darstellen, haben
Sie doch zugleich für viele andere gesprochen)~-- ins
Bewusstsein heben, erlaube ich mir, Ihnen zu schreiben.

Das von Ihnen zuerst behandelte Motiv: Mathematik als
reinste Wissenschaft, als Prototyp unvergänglicher Erkennt\bs
nis, das ist wohl auch im Verlauf der bisherigen Geschichte
--~seit Thales und den Pythagoräern~-- das wirksamste Motiv
gewesen. Gegenwärtig scheint sich dieses Motiv allerdings
in einer besonderen Gefahr zu befinden. Die Geometrie,
die doch bisher --~wie ja offiziell auch heute noch~--
immer zur Mathematik gerechnet wurde, hat seit dem vorigen
Jahrhundert den Charakter der absoluten Sicherheit verloren.
Die Mathematik hat sich daher bezüglich der Geometrie auf
Implikationen der Form: "`wenn die und die Axiome gelten,
dann gilt auch \dots{}"' zurückgezogen, also auf Aussagen, die
kaum noch geometrisch zu heissen verdienen. Wenn ich Sie
nicht missverstanden habe, verstehen Sie unter Mathematik
den engeren Begriff, der nur Logik, Arithmetik und Analysis
umfasst. Neben diesen konkreten Teilen der Mathematik würden
dann die abstrakten Teile --~also die axiomatischen Theorien
der Algebra und Topologie~-- eine sekundäre Rolle spielen.[2]
Will man die Geometrie, eventuell zusammen mit der Mechanik
nicht als ein eigenes Fach konstituieren, so wird man sie
mit zur theoretischen Physik rechnen müssen. Gegenwärtig
wollen nun manche sogar noch der Mathematik im engeren Sinne
die unumstössliche Gültigkeit absprechen, also z.\ B.\ auch die
Arithmetik auf Implikationen: "`wenn die Peano-Axiome gelten,
dann gilt auch \dots{}"' reduzieren.

Dann gäbe es keine Mathematik als Wissenschaft mehr, es gäbe
nur noch formales Ableiten aus Axiomen, die aufgrund pragma\bs
tisch-empirischer Kriterien gewählt werden. Zieht man schliess\bs
lich die Logik mit in diesen Relativierungsprozess hinein,
so würden auch noch die Regeln des formalen Ableitens aus
Axiomen nur durch aussermathematische Kriterien zu
gewinnen sein.

Ich wage, zu vermuten, dass es vor allem diese Gefahr ist,
die Sie als Formalisierung eine inhärente Tragik der Mathe\bs
matik nennen. Hier würde ich mir nun gern die Frage erlauben:
ist diese Formalisierung zu unterscheiden von der "`Formali\bs
sierung"', die in Ihrer Betrachtung über die Bedeutung einer
klaren und prägnanten Bezeichnungsweise als eine Gefahr dar\bs
gestellt wird? Die Existenzaussage auf p.~22 würde nach Er\bs
setzung der logischen Partikeln durch Symbole, nämlich von

\begin{tabular}{@{}llc@{}}%
wenn, so&durch&$\rightarrow$\\%
und&durch&$\land$\\%
es gibt&durch&$\biglor$\\%
ist&durch&$\varepsilon$%
\end{tabular}

lauten:%
\[%
  p\mathrel\varepsilon\mathrm{prim}\land p=4n+1\ \rightarrow\ \biglor\nolimits_{\!\!x,y}\ p=x^2+y^2\ [3]%
\]

Zur "`Formalisierung"' der Eindeutigkeitsaussage könnte

\begin{tabular}{@{}llc@{}}%
es gibt genau ein&durch&$\biglor\limits^1$%
\end{tabular}

ersetzt werden, und wir erhielten dann	%
\[%
  p\mathrel\varepsilon\mathrm{prim}\land p=4n+1\ \rightarrow\ \mathop{\biglor\limits^1}\nolimits_{\!\!x,y}x<y\land p=x^2+y^2%
\]

Wenn man die logischen Symbole nur als prägnante Abkürzung
für die umgangssprachlichen Partikel benutzt --~ihnen also
alle Inhaltlichkeit lässt, und die Aussagen jetzt nicht
plötzlich als bedeutungslose Zeichenreihen behandelt~--
dann scheinen mir genau dieselben Gründe für diese Symbolik zu
sprechen, die uns veranlasst haben, von:

\begin{tabular}{@{}ll@{}}%
  &\llap{"`}$p$ ist die Summe der Quadrate von~$x$ und~$y$"'\\%
  zu&$p=x^2+y^2$%
\end{tabular}

überzugehen. Könnte man der letzten Formel vorwerfen, dass
Sie dem Fluss der suggestiven Sprache Gewalt antut?

Dadurch, dass die logische Symbolik von Hilbert zu dem Zweck
gebraucht ist, eine inhaltliche Theorie in einen axiomatischen
Formalismus zu verwandeln, scheint mir die Möglichkeit
eines inhaltlichen Gebrauches der logischen Symbole zu kurz
gekommen zu sein.

Ich bitte Sie herzlich, diese Bemerkungen nicht als Pro\bs
paganda für die Logistik auffassen zu wollen --~ganz im
Gegenteil, es ist ja gerade die Logistik, die das inhaltliche
Denken verkennt~-- ich würde mich aber freuen, wenn Sie
diesen Brief als einen Ausdruck meiner Dankbarkeit annehmen
wollen, dafür, dass Sie die geistigen Schmerzen eines
"`deutschen Aufsatzes"' nicht gescheut haben, um einmal zur
Besinnung auf unser Tun aufzurufen.\strut\medskip

\begin{tabular}{@{}rl@{}}%
  Mit den ergebensten Grüssen bin ich&\\%
  Ihr&\\%
  &P. L.%
\end{tabular}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

